Leveraging Clinical Context for User-Centered Explainability: A Diabetes Use Case

Academic advances of AI models in high-precision domains, like healthcare, need to be made explainable in order to enhance real-world adoption. Our past studies and ongoing interactions indicate that medical experts can use AI systems with greater trust if there are ways to connect the model inferences about patients to explanations that are tied back to the context of use. Specifically, risk prediction is a complex problem of diagnostic and interventional importance to clinicians wherein they consult different sources to make decisions. To enable the adoption of the ever improving AI risk prediction models in practice, we have begun to explore techniques to contextualize such models along three dimensions of interest: the patients' clinical state, AI predictions about their risk of complications, and algorithmic explanations supporting the predictions. We validate the importance of these dimensions by implementing a proof-of-concept (POC) in type-2 diabetes (T2DM) use case where we assess the risk of chronic kidney disease (CKD) - a common T2DM comorbidity. Within the POC, we include risk prediction models for CKD, post-hoc explainers of the predictions, and other natural-language modules which operationalize domain knowledge and CPGs to provide context. With primary care physicians (PCP) as our end-users, we present our initial results and clinician feedback in this paper. Our POC approach covers multiple knowledge sources and clinical scenarios, blends knowledge to explain data and predictions to PCPs, and received an enthusiastic response from our medical expert.

==> expert_feedback.tex <==
% mainfile: main.tex

Our work, and in particular this POC, was advised and evaluated by a clinical researcher, who is also a clinician by training. Our use case was designed for clinical relevance (such as the time horizon for CKD prediction) in consultation with the expert. Overall, the expert opined that our approach holds potential to contextualize, or connect relevant clinical information, to help clinicians make informed decisions about the various entities that they generally interact with when they are treating patients.
They also evaluated the three dimensions of contextualization we addressed to be of high value. Specifically, the set of questions was evaluated to be of relevance to the clinical workflow. Similarly, the contextualization of the important features, using the medical ontology, followed their advice and we intend to further explore {\dm} groupings in the future. 
The expert evaluation also points to several areas where we can improve the POC, such as increasing the persona coverage beyond PCPs, providing more in-depth contextualization, and supporting more presentation styles to present the results in a more clinically relevant manner. 
We intend to address these in our full paper. Specifically, our ongoing work is focused on using the patient's context to probe guidelines and create question lists for various types of clinicians (such as PCPs and endocrinologists with more in-depth knowledge). We are also exploring the possibility of adding more points of contextualization (such as extracting richer content from guidelines) and leveraging other augmentation sources, such as biomedical ontologies.

Overall, the expert's feedback validates our long-terms goals to make the explanations more adaptive to the end-user's expertise and situate them in the context of the patients they see. 
Our described approach enables contextualization for clinical use cases across three specific dimensions that aim to generate user-centered explanations that can help clinicians make knowledge-enabled decisions. We are in the process of building a prototype dashboard and conducting a full scale user study to evaluate the importance of our proposed solution.

%To include more presentation styles that would mimic clinicians in their reasoning process, we plan to develop modules to present information in our previously identified literature-derived explanation types that capture various aspects (e.g. contrastive, counterfactual, evidence-based explanations). 

\iffalse
%Pablo This can be reduced a bit
%SC Share the conclusions and not the process
During our design and evaluation stage of the methodology presented, we engaged with a clinical researcher who is also a clinician by training. 
%SC commenting for process
% We conducted collaborative walkthrough sessions with the expert at different stages of design and evaluation.
The expert believes that our approach holds potential to contextualize, or provide relevant information, to help clinicians make informed decisions about the various entities that they generally interact with when they are treating patients. With this belief, they provided suggestions to make our approach more clinically relevant and useful, and we accommodated some of the expert's suggestions within the presented POC and are planning to address the rest in the next iteration of the pipeline. 
%SC Share a higher-level summary - be less quantitative 
Specifically, we increased the time horizon for CKD prediction based on how often clinicians typically see CKD manifestations in T2D patients and what is a typical window for any actionable insights using the model.
%SC Changed symptoms to manifestations based on Fernando's feedback
The expert also suggested that certain questions would be more clinically relevant
% SC to clinicians,
%SC commented above based on Fernando's comment
, and we prioritized these as shown under Sec \ref{sec:results}. 
With respect to the feature importance (see Fig. \ref{fig:shap:bar_proto}), the expert recommended to introduce meaningful groupings, e.g., to group together complications of T2D and present them in a hierarchical manner (also emphasized as one of the explainable AI strategies in~\cite{lecue2020role}). We used top-level CCS codes to situate the lower level diagnoses codes seen in the patient data (seen in Fig. \ref{fig:shap:summary_proto} and Table \ref{tab:resultsquestions}), and we are investigating resources that can aid us for T2D groupings.
% \explannote[SC]{PC can edit the above depending on if the classifications are included.}

The suggestions we are planning to address in the future are towards increasing coverage capabilities, and supporting more presentation styles to present the results in a more clinically relevant manner. In terms of increasing coverage, we were recommended and plan to use the patient's context to probe guidelines, create question lists for various types of clinicians (e.g., PCPs, endocrinologists with more in-depth knowledge), and include more points of contextualization. Specifically, we plan to consider contextualization points, i.e., to include more content from guidelines besides just the recommendations and leverage other augmentation sources such as biomedical ontologies (e.g., the disease and drug ontologies). To include more presentation styles that would mimic clinicians in their reasoning process, we plan to develop modules to present information in our previously identified literature-derived explanation types that capture various aspects (e.g., contrastive, counterfactual, evidence-based explanations). 

In summary, the expert's feedback which aligns with our overall goals is to make the explanations more adaptive to the end-user's expertise and situate them in the context of the patients they see. Overall, our described approach that enables contextualization in a clinical, T2DM use case, along the dimensions of AI model predictions, post-hoc explanations for patients and patients themselves via user-centered explanations would help clinicians make knowledge-enabled decisions. 

\fi
